Explaining GitHub Actions Failures with Large Language Models: Challenges, Insights, and Limitations

GitHub Actions (GA) has become the de facto tool that developers use to automate software workflows, seamlessly building, testing, and deploying code. Yet when GA fails, it disrupts development, causing delays and driving up costs. Diagnosing failures becomes especially challenging because error logs are often long, complex and unstructured. Given these difficulties, this study explores the potential of large language models (LLMs) to generate correct, clear, concise, and actionable contextual descriptions (or summaries) for GA failures, focusing on developers' perceptions of their feasibility and usefulness. Our results show that over 80\% of developers rated LLM explanations positively in terms of correctness for simpler/small logs. Overall, our findings suggest that LLMs can feasibly assist developers in understanding common GA errors, thus, potentially reducing manual analysis. However, we also found that improved reasoning abilities are needed to support more complex CI/CD scenarios. For instance, less experienced developers tend to be more positive on the described context, while seasoned developers prefer concise summaries. Overall, our work offers key insights for researchers enhancing LLM reasoning, particularly in adapting explanations to user expertise.

==> body_text/3_RQ1_results.tex <==
\section{Correctness (RQ1)}


 
\begin{figure}[t]
\raggedleft
\includegraphics[scale=0.58 ]{figures/rq1_results.pdf}
\caption{The stacked bar chart shows the levels of agreement of participants to our statements

\ref{st:one}, \ref{st:three}, \ref{st:four}, \ref{st:five}, and \ref{st:six}.}
\label{fig:rq1_results}
\end{figure}

To address RQ1, we analyzed developer responses to statements \ref{st:one}, \ref{st:three}, \ref{st:four}, \ref{st:five}, and \ref{st:six}, which evaluate distinct aspects of the \emph{correctness} of LLM explanations. 

Overall, developers rated the correctness of LLM-generated explanations as high for all these statements (see Fig.~\ref{fig:rq1_results}). St. \ref{st:one}, which evaluated whether the explanations accurately reflected the details and context of the GA run failures, received a mean score of 4.39, with 83\% of participants agreeing. St. \ref{st:three}, which assessed the likelihood of the explanations not containing misleading content, achieved a mean score of 4.03, with 77\% of participants expressing low concern for misleading information. St. \ref{st:four}, focusing on the accuracy of diagnosing technical aspects of the failure, received a mean score of 4.31, with 78\% of participants in agreement. St. \ref{st:five}, which evaluated the absence of incorrect content, recorded a mean score of 4.31, with 84\% agreement among participants. Finally, St. \ref{st:six}, assessing the logical soundness of the explanations, received a mean score of 4.31, with a high agreement rate of 87\% among participants.
 




\begin{tcolorbox}[colback=gray!5!white, colframe=gray!75!black, title=  Answer to RQ1]
In summary, developers generally rated the \emph{correctness} of LLM-generated explanations as high, with over 80\% agreeing that these explanations accurately captured essential details and effectively diagnosed GA run failures. The explanations were perceived as factually reliable and logically coherent, supporting their usefulness  to improve the GA failure
management process.
\end{tcolorbox}


==> body_text/backup/2_study_design_aRQ.tex <==
\section{Study Design}

The goal of this study, framed by the overarching question \emph{Can Large Language Models Explain GitHub Action Failures?} is to evaluate the feasibility of using LLMs not only to explain GA run failures and gain insights into developers' needs when interpreting error logs. Specifically, we aim to evaluate how developers perceive the accuracy with which LLMs capture the details and context of run failures (performance expectancy – accuracy), the clarity of the explanations (effort expectancy – clarity), and the usefulness of these explanations in offering actionable insights that make error explanations effective for troubleshooting (performance expectancy – usefulness).


We define three research questions that guide our study.

\noindent \textbf{RQ1: To what extent do developers believe that Large Language Models accurately capture the specific details and context of run failures in their explanations?}


This research question examines how developers perceive the accuracy of LLM-generated explanations in capturing the details and context of GitHub Actions run failures, focusing on performance expectancy – accuracy. Accuracy here encompasses more than just technical correctness; it reflects how well the explanations align with developers' practical experience and understanding. Developers need specific, context-aware information to diagnose issues effectively. Omission of critical details or overly general explanations from LLMs could impair rather than enhance the troubleshooting process. This question evaluates whether LLMs provide insights that meet developers' expectations, ensuring explanations are not only technically accurate but also contextually relevant and practically useful for resolving issues in real-world scenarios.


\noindent \textbf{RQ2: To what extent do developers find the explanations provided by Large Language Models for GitHub Actions run failures clear and useful?}

Clarity and usefulness are important factors in ensuring that LLM-generated explanations are understandable and actionable for developers. Clear explanations help developers interpret system behavior and diagnose issues more easily, while usefulness reflects whether the explanations offer practical steps for addressing run failures. This research question examines participants' evaluations, exploring how well LLM-generated explanations meet these criteria, with a focus on making sure that explanations are not only accurate but also accessible and helpful for developers.


\noindent \textbf{RQ3: What attributes make an error explanation effective to addressing issues related to GitHub Actions run failures?}

Identifying the attributes that contribute to an explanation’s  effectiveness—whether it involves brevity, detailed steps, or actionable insights—aligns with performance expectancy – usefulness. Understanding these factors can inform how LLMs are integrated into the diagnostic process, ensuring that their explanations are tailored to meet developers' needs. This research question explores which qualities enhance the practical value of LLM-generated explanations, helping to refine their application in ways that improve troubleshooting efficiency and developer satisfaction.


To address the three research questions, we conducted a survey among GA developers (Section~\ref{sec:Survey}). The collected data was analyzed using a combination of quantitative and qualitative analysis (Section~\ref{sec:Analysis}). Materials to support the replication of this work are provided as supplemental materials~\cite{reference}.


==> body_text/backup/DSAC.tex <==

\subsection{Data Analysis}\label{sec:Analysis}

To analyze the data, we employed a combination of quantitative and qualitative techniques. This approach was necessary because our survey included both closed-ended statements and open-ended questions that allowed for detailed, free-form responses. The question formats and response options were informed by results from a survey pilot as well as prior studies on human evaluations of AI programming assistants (e.g.,~\cite{barke2023grounded,cheng2024would,dakhel2023github,denny2023conversing,imai2022github,jayagopal2022exploring,jiang2022discovering}).

\emph{Quantitative Analysis.} We followed best practices for survey data analysis as outlined by Kitchenham and Pfleeger \cite{kitchenham2008personal} to conduct our quantitative analysis for RQ1 and RQ2.

To address RQ1, we analyze responses to statements 1, 4, 5, and 6 from the survey, which were selected to directly evaluate how developers perceive the correctness and content adequacy of LLM-generated explanations for GitHub Actions run failures.


\begin{itemize}
    \item \emph{St. 1} evaluates \emph{content adequacy}, examining whether the explanation captures the essential details and context of the failure, providing the necessary information for effective troubleshooting.

    \item \emph{St. 4} assesses \emph{correctness}, determining whether the explanation accurately identifies and diagnoses the cause of the failure.


    \item \emph{St. 5} evaluates \emph{correctness} by checking for the presence of incorrect or irrelevant content, ensuring that the explanation is trustworthy.


    \item \emph{St. 6} assesses \emph{content adequacy}, focusing on the soundness of the diagnostic reasoning provided, which aids developers in connecting the explanation to actionable insights.


\end{itemize}

We compute descriptive statistics (mean, median, standard deviation) for these statements to capture central tendencies and variability in participants' responses. This analysis helps quantify how well developers perceive the LLM explanations align with their practical experience, ensuring the explanations are both accurate and contextually relevant, as discussed by Henricksen  \etal~\cite{henricksen2005modelling}.

For RQ2, we analyze responses to statements 2, 3, 7, 8, 9, and 10, which assess the conciseness and expressiveness of LLM-generated explanations for GitHub Actions run failures. Expressiveness refers to how clearly the explanations communicate information, while conciseness reflects whether the explanations provide the necessary details without unnecessary information, ensuring they are actionable and efficient.



\begin{itemize}
    \item \emph{St. 2} evaluates \emph{conciseness}, determining how efficiently the explanation guides developers toward resolving the failure without including excessive information.

    \item \emph{St. 3} examines \emph{conciseness}, assessing the likelihood of the explanation containing misleading or irrelevant information that could reduce its clarity or usefulness.

    \item \emph{St. 7} focuses on \emph{expressiveness}, evaluating whether the explanation communicates the run failure clearly, ensuring it is easy for developers to interpret.

    \item \emph{St. 8} considers \emph{expressiveness}, analyzing whether the explanation outlines the subsequent steps in a clear and actionable manner.

    \item \emph{St. 9} assesses \emph{conciseness}, evaluating how well the explanation addresses the specific needs of developers without being overly general or vague.

    \item \emph{St. 10} addresses \emph{expressiveness}, examining developers' confidence in the diagnosis, ensuring that the explanation not only describes the failure but also inspires trust in the proposed solution.


\end{itemize}

We compute descriptive statistics (mean, median, standard deviation) to capture how participants assess the clarity and practical value of the explanations. This analysis reveals how well LLM explanations meet developers' expectations for clear, useful, and actionable guidance, enabling them to diagnose run failures.


\emph{Qualitative Analysis.} To address RQ3, we applied open coding \cite{charmaz2014constructing} followed by a card sorting analysis \cite{zimmermann2016card} on the open-ended responses from survey questions 11 and 12. This analysis aimed to identify the key attributes that make an LLM-generated explanation actionable and effective for resolving GitHub Actions run failures. Attributes such as conciseness, expressiveness, and the inclusion of actionable steps were highlighted as critical for making explanations more useful in practice. Understanding these factors helps refine LLM-generated explanations to better align with developers' expectations and needs. The goal is to ensure that the explanations provided by LLMs not only help developers diagnose issues more efficiently but also offer clear, concise, and actionable insights that directly support the resolution of run failures.



==> figures/table.tex <==
% \usepackage{booktabs}


\begin{table}
    \centering
    \begin{tabular}{llll} 
    \toprule
    questions
      title                                                                                & \% Agreement & Average Score & Conflict Factor  \\ 
    \midrule
    I am confident in the diagnosis provided
      by the run failure explanation.                       & 79.38        & 4.15          & 9.07             \\
    The run failure explanation is helpful.                                                          & 82.81        & 4.28          & 10.6             \\
    The explanation specifically addresses my
      needs without feeling too general.                   & 76.56        & 4.08          & 7.66             \\ 
    \hline\hline
    The explanation accurately diagnoses the
      run failure.                                          & 81.56        & 4.27          & 12.43            \\
    The explanation accurately reflects the
      details and context of the GitHub Actions run failure. & 86.56        & 4.39          & 18.47            \\
    The explanation clearly and
      understandably communicates the run failure.                       & 82.5         & 4.29          & 11.48            \\ 
    \hline\hline
    There is evident sound diagnostic
      reasoning.                                                   & 81.25        & 4.29          & 14.44            \\
    The explanation clearly outlines the
      following steps to take.                                  & 82.19        & 4.3           & 15.47            \\ 
    \hline\hline
    The explanation contains no inappropriate
      or incorrect content.                                & 78.75        & 4.3           & 19.38            \\
    There is a low likelihood of a possible
      misleading explanation.                                & 73.75        & 4.01          & 6.94             \\
    \hline
    \end{tabular}
    \end{table}

==> tables/table_developers_profiles.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.5} % Ajusta la altura de las filas
\centering
\caption{Profiles of Developers Involved in the Study.}
\begin{tabular}{p{5cm} >{\raggedleft\arraybackslash}p{2cm}} 
\toprule
\textbf{Attribute} & \textbf{Proportion (\%)} \\ 
\midrule
\multicolumn{2}{l}{\textbf{Gender}} \\
Male & 90.32\% \\
Female & 9.68\% \\
\midrule
\multicolumn{2}{l}{\textbf{Professional experience}} \\
None & 3.23\% \\
1 year or less & 6.45\% \\
2 years & 12.90\% \\
3-5 years & 9.68\% \\
6-10 years & 16.13\% \\
11+ years & 51.61\% \\
\midrule
\multicolumn{2}{l}{\textbf{Educational Level}} \\
High school graduate or GED & 3.23\% \\
Some college or 2-year degree & 3.23\% \\
Bachelor in Computer Science/Software Engineering & 22.58\% \\
Bachelor in other STEM fields & 16.13\% \\
Master in Computer Science & 38.71\% \\
Master in other STEM fields & 6.45\% \\
Master in non-STEM fields & 6.45\% \\
PhD or other advanced degrees & 3.23\% \\
\bottomrule
\end{tabular}
\label{table:developer_profiles}
\end{table}

==> tables/table_rq1.tex <==
\begin{table*}[htbp]
\centering
\vspace{1cm} 
\caption{Descriptive Statistics for Accuracy-Related Statements.}
\label{tab:descriptive_stats_graphs}
% \small
\begin{tabularx}{\textwidth}{p{0.31\textwidth} p{0.02\textwidth} p{0.03\textwidth} p{0.04\textwidth} | p{0.6\textwidth}}
\toprule
\textbf{Statement} & \textbf{Mean} & \textbf{Median} & \textbf{Std. Dev.} & \textbf{Graph} \\ 
\midrule
The explanation accurately reflects the details and context of the GitHub Actions run failure.  & 4.39 & 5.0 & 0.89 & \multirow{4}{*}{\includegraphics[width=8cm,height=2.6cm]{figures/group1.png}} \\ 
The explanation accurately diagnoses the run failure.  & 4.31 & 5.0 & 0.96 & \\
The explanation contains no inappropriate or incorrect content.  & 4.31 & 5.0 & 0.97 & \\
There is evident sound diagnostic reasoning.  & 4.31 & 5.0 & 0.93 & \\
\midrule
\end{tabularx}

% Legend
\begin{tabularx}{\textwidth}{XXXXX}
\makebox[2em][c]{\colorbox{fullyagree}{\rule{0pt}{0.6em}}} Fully Agree & 
\makebox[2em][c]{\colorbox{agree}{\rule{0pt}{0.6em}}} Agree & 
\makebox[2em][c]{\colorbox{neutral}{\rule{0pt}{0.6em}}} Neutral & 
\makebox[2em][c]{\colorbox{disagree}{\rule{0pt}{0.6em}}} Disagree & 
\makebox[2em][c]{\colorbox{stronglydisagree}{\rule{0pt}{0.6em}}} Strongly Disagree \\
\bottomrule
\end{tabularx}
\end{table*}

==> tables/table_rq1_v2.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\small % Reduce font size
\label{tab:rq1_desc}

\caption{RQ1 Statements and Results \pv{table format will be update}}
\begin{tabular}{|c|p{2.8cm}|c|c|c|c|c|c|c|c|}
\hline
\textbf{No.} & \textbf{Statement} & \textbf{Mean} & \textbf{Median} & \textbf{Std. Dev.} & \textbf{Fully Agree} & \textbf{Agree} & \textbf{Neutral} & \textbf{Disagree} & \textbf{S. Disagree} \\
\hline
1 & The explanation accurately reflects the details and context of the GitHub Actions run failure. & 4.39 & 5 & 0.89 & 50 & 32.6 & 11.6 & 3.9 & 1.9 \\
\hline
3 & There is a low likelihood of a misleading explanation. & 4.03 & 4 & 1.15 & 45 & 32.4 & 10.5 & 6.1 & 5.0 \\
\hline
4 & The explanation accurately diagnoses the run failure. & 4.31 & 5 & 0.96 & 48 & 30.4 & 16.3 & 3.2 & 2.1 \\
\hline
5 & The explanation contains no inappropriate or incorrect content. & 4.31 & 5 & 0.97 & 56 & 27.5 & 9.7 & 4.2 & 2.6 \\
\hline
6 & There is evident sound diagnostic reasoning. & 4.31 & 5 & 0.93 & 54 & 33.1 & 7.1 & 4.1 & 1.7 \\
\hline
\end{tabular}
\end{table*}



==> tables/table_rq2.tex <==
\begin{table*}[t]
\centering
\vspace{1cm} 
\caption{Descriptive Statistics for Clarity and Usefulness-Related Statements.}
\label{tab:descriptive_stats_graphs}
% \small
\begin{tabularx}{\textwidth}{p{0.31\textwidth} p{0.02\textwidth} p{0.03\textwidth} p{0.04\textwidth} | p{0.6\textwidth}}
\toprule
\textbf{Statement} & \textbf{Mean} & \textbf{Median} & \textbf{Std. Dev.} & \textbf{Graph} \\ 
\midrule
The run failure explanation is helpful. & 4.30 & 5.0 & 1.01 & \multirow{4}{*}{\includegraphics[width=8cm,height=3.5cm]{figures/group2.png}} \\ 
There is a low likelihood of a possible misleading explanation. & 4.03 & 4.0 & 1.15 & \\
The explanation clearly and understandably communicates the run failure. & 4.31 & 5.0 & 0.96 & \\
The explanation clearly outlines the following steps to take. & 4.33 & 5.0 & 0.94 & \\
The explanation specifically addresses my needs without feeling too general. & 4.11 & 4.0 & 1.06 & \\
I am confident in the diagnosis provided by the run failure explanation. & 4.18 & 4.0 & 1.05 & \\
\bottomrule
\multicolumn{5}{c}{\includegraphics[width=11cm,height=1.5cm]{figures/legend.png}} \\
\end{tabularx}
 
\end{table*}

==> tables/table_rq2_v2.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\small % Reduce font size
\label{tab:rq2_desc}

\caption{RQ2 Statements and Results}
\begin{tabular}{|c|p{3.5cm}|c|c|c|c|c|c|c|c|}
\hline
\textbf{No.} & \textbf{Statement} & \textbf{Mean} & \textbf{Median} & \textbf{Std. Dev.} & \textbf{Fully Agree} & \textbf{Agree} & \textbf{Neutral} & \textbf{Disagree} & \textbf{Strongly Disagree} \\
\hline
2 & The run failure explanation is helpful. & 4.3 & 5 & 1.01 & 50 & 30.3 & 9.7 & 5.0 & 5.0 \\
\hline
5 & The explanation contains no inappropriate or incorrect content. & 4.31 & 5 & 0.97 & 56 & 27.5 & 9.7 & 4.2 & 2.6 \\
\hline
7 & The explanation clearly and understandably communicates the run failure. & 4.31 & 5 & 0.96 & 48 & 34.6 & 10.6 & 4.8 & 2.1 \\
\hline
8 & The explanation clearly outlines the subsequent steps to take. & 4.33 & 5 & 0.94 & 54 & 28.9 & 12.9 & 2.7 & 1.7 \\
\hline
9 & The explanation specifically addresses my needs without feeling too general. & 4.11 & 4 & 1.06 & 42 & 32.5 & 11.3 & 8.4 & 5.3 \\
\hline
10 & I am confident in the diagnosis provided by the run failure explanation. & 4.18 & 4 & 1.05 & 45 & 38.2 & 10.5 & 5.7 & 3.6 \\
\hline

\end{tabular}
\end{table*}


==> tables/table_taxonomy.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row height
\caption{Taxonomy of attributes that make an explanation useful for addressing GitHub Actions run failures. \todo{will be updated}}
\label{table:taxonomy}
\begin{tabular}{m{3.5cm} m{5cm} m{6cm}}
\toprule
\textbf{Main Category} & \textbf{Specific Attributes} & \textbf{Example Sentence} \\
\midrule
\multirow{3}{3.5cm}{Clarity of the Explanation (28\%)} 
 & Clarity in Error Explanation & \emph{``The explanation in the survey looks good enough from a general knowledge perspective.''} \\
 & Clarity in Steps to Follow & \emph{``Cutting fluff, going straight to the point. Possible steps to take to fix the problem.''} \\
\midrule
\multirow{3}{3.5cm}{Actionable Guidance (30\%)} 
 & Precision in Instructions & \emph{``I believe that a useful error explanation should get straight to the point without saying a lot of unnecessary things.''} \\
 & Direct Applicability of Suggested Steps & \emph{``The most valuable part of an error explanation is detailing what the error message means in simple, plain-English terms.''} \\
\midrule
\multirow{2}{3.5cm}{Specificity of Content (18\%)} 
 & Adaptation of content to the context of the failure & \emph{``Detecting the right context is key for error detection.''} \\
 & Technical accuracy in describing the problem & \emph{``It helps developers that are 'consuming' tests to figure out where the failure happened and why.''} \\
\midrule
\multirow{3}{3.5cm}{Contextual Relevance (13\%)} 
 & Inclusion of relevant links & \emph{``Concise information with links to relevant GitHub Actions documentation, issue trackers, or other resources that provide more in-depth information.''} \\
 & Explicit mention of dependencies or technical conflicts & \emph{``Referencing components explicitly. E.g. saying there is a dependency conflict between lib X and lib Y.''} \\
\midrule
\multirow{3}{3.5cm}{Conciseness (11\%)} 
 & Ability to quickly summarize the cause of the failure & \emph{``The explanation got straight to the point and identified the root cause quickly.''} \\
 & Concise Presentation of Resolution Steps & \emph{``Brief and concise explanation, with specific steps to be followed.''} \\
\bottomrule
\end{tabular}
\end{table*}

